Robust Models are less Over-Confident

Despite the success of convolutional neural networks (CNNs) in many academic benchmarks for computer vision tasks, their application in the real-world is still facing fundamental challenges. One of these open problems is the inherent lack of robustness, unveiled by the striking effectiveness of adversarial attacks. Current attack methods are able to manipulate the network's prediction by adding specific but small amounts of noise to the input. In turn, adversarial training (AT) aims to achieve robustness against such attacks and ideally a better model generalization ability by including adversarial samples in the trainingset. However, an in-depth analysis of the resulting robust models beyond adversarial robustness is still pending. In this paper, we empirically analyze a variety of adversarially trained models that achieve high robust accuracies when facing state-of-the-art attacks and we show that AT has an interesting side-effect: it leads to models that are significantly less overconfident with their decisions, even on clean data than non-robust models. Further, our analysis of robust models shows that not only AT but also the model's building blocks (like activation functions and pooling) have a strong influence on the models' prediction confidences. Data & Project website: https://github.com/GeJulia/robustness_confidences_evaluation

==> activation_cifar10.tex <==
\begin{figure}
 \tiny
\begin{center}

\begin{tabular}{c}
\begin{minipage}{0.9\columnwidth}
      \includegraphics[width=\linewidth]{figures/confi_curves_normal_Carmon2019Unlabeled.pdf}
     \end{minipage}  
  \\
  \begin{minipage}{0.9\columnwidth}
      \includegraphics[width=\linewidth]{figures/confi_curves_robust_Dai2021Parameterizing.pdf}
     \end{minipage}  
  \\ 
  \begin{minipage}{0.9\columnwidth}
      \includegraphics[width=\linewidth]{figures/confi_curves_robust_Carmon2019Unlabeled.pdf}
     \end{minipage}  
 \\ \end{tabular}


 \caption[]{Confidence distribution on three different WRN-28-10. The first row shows a model without adversarial training and standard activation (ReLu), the second row the model by \citet{dai2021parameterizing} which uses learnable activation functions instead of fixed ones and the third row shows the model by \citet{carmon2019unlabeled} adversarially trained and with the standard activation (ReLu).}
 \label{fig:activation_cifar10}
 \end{center}
 \end{figure}

==> cifar100_roc_neurips.tex <==
\begin{figure}
 \tiny
\begin{center}

\begin{tabular}{ccc}

  \begin{minipage}{.32\columnwidth}
      \includegraphics[width=\linewidth]{figures/mean_auc_robust_all_cifar100_Clean_pgd.pdf} 
      \end{minipage}
       
&
  \begin{minipage}{.32\columnwidth}
      \includegraphics[width=\linewidth]{figures/mean_auc_robust_all_cifar100_Adv_pgd.pdf}
     \end{minipage}  
     &
     \begin{minipage}{.32\columnwidth}
      \includegraphics[width=\linewidth]{figures/mean_auc_robust_all_cifar100_Adv_squares.pdf}
     \end{minipage}  
     \\ &
     \\ \multicolumn{3}{c}{
\begin{minipage}{.7\columnwidth}
      \includegraphics[width=\linewidth]{auc_legend_neurips.pdf}
     \end{minipage} }
  \\
 \end{tabular}

 \caption[]{Average ROC curve for all robust and all non-robust models trained on CIFAR100. Standard deviation is marked by the error bars. The dashed line would mark a model which has the same confidence for each prediction. We can clearly see that the models confidences can be an indicator for the correctness of the prediction. However, on PGD samples the non-robust models fail completely while the robust models are still able to distinguish correct from incorrect predictions based on the prediction confidence.}
 \label{fig:roc_cifar100}
 \end{center}
 \end{figure}

==> cifar100_scatter.tex <==
\begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\textwidth]{figures/pretty_scatter_confi_acc_cifar100.pdf}}
\caption{Mean model confidences on their correct (x-axis) and incorrect (y-axis) predictions over 1000 samples of the CIFAR100 dataset clean and perturbated with PGD and Squares. Each point represents a model. Circular points (purple color-map) represent non-robust models and diamond-shaped points (green color-map) represent robust models. The color of each point represents the models accuracy, darker signifies higher accuracy (better) on the given data samples (clean or perturbated). The star in the bottom right corner symbolizes the optimal model and the gray area marks the area were the confidence distribution of the network is worse Concretely, we penalize for high confidences on incorrect predictions and reward for high confidence on correct predictions.}
\label{fig:confi_all_cifar100}
\end{center}
\vskip -0.2in
\end{figure*}

==> ece_imagenet.tex <==
\begin{figure*}[ht]
 \tiny
\begin{center}

\begin{tabular}{cc}
\large{Clean Samples}  \\
\begin{minipage}{.49\textwidth}
      \includegraphics[width=\linewidth]{ece_bar_plot_clean_imagenet.pdf}
     \end{minipage}  
     &
     \begin{minipage}{.49\textwidth}
      \includegraphics[width=\linewidth]{ece_legend_imagnet.pdf}
     \end{minipage}  
 \\
 \large{PGD Samples} & \large{Squares} \\
  \begin{minipage}{.49\textwidth}
      \includegraphics[width=\linewidth]{ece_bar_plot_pgd_imagenet.pdf}
     \end{minipage}  
& 
  \begin{minipage}{.49\textwidth}
      \includegraphics[width=\linewidth]{ece_bar_plot_squares_imagenet.pdf}
     \end{minipage}  
 \end{tabular}
 \\
 \caption[]{ECE (lower is better) bar plots of the models trained on ImageNet provided by RobustBench \cite{robust_bench}. The non-robust baseline exhibits the worst ECE. In contrast, the robust models are better calibrated. }
 \label{fig:ece_imagenet}
 \end{center}
 \end{figure*}

